A brief overview of programmed instructions for quantum software education

In this paper we provide an overview of the programmed instructions approach for the purpose of quantum software education. The article presents the programmed instructions method and recent successes in STEM fields before describing its operating mode. Elements tackled include the core components of programmed instructions, its behavioural roots and early use as well as adaptation to complex STEM material. In addition, we offer recommendations for its use in the specific context of quantum software education and provide one example of PI-based instruction for the notion of entanglement. The aim of this work is to provide high-level guidelines for incorporating programmed instructions in quantum education with the goal of disseminating quantum skills and notions more efficiently to a wider audience.

==> sections/current_quantum_educ_approaches.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A glimpse into the quantum education landscape}

The last century has seen the number of teaching approaches soar in education. From the teacher-centered didactic instruction to Montessori \cite{dohrmann2007high} by way of inquiry-based and constructivism, knowledge flow has received considerable attention. However, the further away one goes from primary school to higher education, the less likely it is that the teaching method differs from the widespread \textit{lecture-style didactic teaching}. 

As detailed in the excellent review by Kaur \textit{et.al.}\cite{kaur2022defining} the current quantum education landscape offers a wide variety of resources and approaches. Industry and academia \cite{aiello2021achieving} have put considerable effort into content creation, striving to make quantum education available to a growing audience of non-specialists and early-stage learners \cite{temporao2022teaching}. However, to the best of our knowledge, no quantum educational resources rely clearly on PI so far. Based on the strong evidence of success of PI approaches in STEM fields \cite{kurbanoglu2006programmed, harrington1999teaching, stanisavljevic2013application, Hui2009-kr, emurian2000learning}, its exploitation in QEd appears to be a promising avenue to explore.



